Blockchain Meets LLMs: A Living Survey on Bidirectional Integration

In the domain of large language models, considerable advancements have been attained in multimodal large language models and explainability research, propelled by the continuous technological progress and innovation. Nonetheless, security and privacy concerns continue to pose as prominent challenges in this field. The emergence of blockchain technology, marked by its decentralized nature, tamper-proof attributes, distributed storage functionality, and traceability, has provided novel approaches for resolving these issues. Both of these technologies independently hold vast potential for development; yet, their combination uncovers substantial cross-disciplinary opportunities and growth prospects. The current research tendencies are increasingly concentrating on the integration of blockchain with large language models, with the aim of compensating for their respective limitations through this fusion and promoting further technological evolution. In this study, we evaluate the advantages and developmental constraints of the two technologies, and explore the possibility and development potential of their combination. This paper primarily investigates the technical convergence in two directions: Firstly, the application of large language models to blockchain, where we identify six major development directions and explore solutions to the shortcomings of blockchain technology and their application scenarios; Secondly, the application of blockchain technology to large language models, leveraging the characteristics of blockchain to remedy the deficiencies of large language models and exploring its application potential in multiple fields.

==> Conclusion/conclusion.tex <==
This review provides a summary of the current impact between blockchain and LLMs. In order to better reflect the relationship between blockchain and LLMs, we summarise the advantages and disadvantages of blockchain and LLMs, as well as examples of how each has been used in the other's domain. We hope that this review will give readers a better understanding of the current situation of blockchain and LLMs, and contribute to the future exploration of this area. 


==> Introduction/abstract.tex <==
\paragraph{abstract:In the domain of large language models, considerable advancements have been attained in multimodal large language models and explainability research, propelled by the continuous technological progress and innovation.   Nonetheless, security and privacy concerns continue to pose as prominent challenges in this field.   The emergence of blockchain technology, marked by its decentralized nature, tamper-proof attributes, distributed storage functionality, and traceability, has provided novel approaches for resolving these issues.   Both of these technologies independently hold vast potential for development;   yet, their combination uncovers substantial cross-disciplinary opportunities and growth prospects.   The current research tendencies are increasingly concentrating on the integration of blockchain with large language models, with the aim of compensating for their respective limitations through this fusion and promoting further technological evolution.   In this study, we evaluate the advantages and developmental constraints of the two technologies, and explore the possibility and development potential of their combination.   This paper primarily investigates the technical convergence in two directions: Firstly, the application of large language models to blockchain, where we identify six major development directions and explore solutions to the shortcomings of blockchain technology and their application scenarios;   Secondly, the application of blockchain technology to large language models, leveraging the characteristics of blockchain to remedy the deficiencies of large language models and exploring its application potential in multiple fields.}

==> Technical_advantages/Application_in_smart_contract_auditing/Application_in_smart_contract_auditing.tex <==
\subsection{Application in smart contract auditing}
In today's era of rapid digitalization and intelligence, the integration of blockchain and large language models has become a hot topic in the technology field. Among them, their application in smart contract auditing is of great significance, not only improving the security and reliability of smart contracts, but also promoting the application and development of blockchain technology in wider fields. Next, we will discuss in detail the specific application and development process of blockchain and large language models in smart contract auditing.

\subsubsection{Automatically generate verifiable smart contract code through natural language}
 
.

\subsubsection{Combine LLM’s code verification mechanism to reduce vulnerabilities}
 
In the context that security vulnerabilities in smart contracts have always been a problem in the blockchain field, traditional code audit methods have shortcomings. The development of large language models provides new ideas for smart contract code verification. "CIPHER: Comprehensive Inline Assembly and Solidity Detection for Enhanced Smart Contract Security"\cite{34}proposes a comprehensive inline assembly and Solidity detection method that can detect various vulnerabilities in smart contracts, including reentrancy attacks and integer overflows and permission control issues, etc., and introduces its design and implementation, verifies its effectiveness through experiments, and discusses limitations and improvement directions.In "Securify: Practical security analysis of smart contracts"\cite{35}, Securify, as a practical smart contract security analysis tool, uses static analysis technology to automatically detect security vulnerabilities, provide detailed reports and repair suggestions, and introduces the working principle. and technical implementation, the effectiveness and practicality are verified through the analysis of a large number of real smart contracts, and the challenges and future development directions of smart contract security analysis are also discussed. Researchers apply LLM to smart contract code verification, detect potential security vulnerabilities and provide repair suggestions through semantic analysis and vulnerability pattern recognition, and combine with blockchain distributed ledger technology to achieve real-time monitoring and auditing. Currently, this mechanism has achieved certain results, but it still faces accuracy, reliability and compatibility challenges. In the future, the LLM algorithm and model need to be optimized to improve performance.

\subsubsection{Optimize LLM’s code generation capabilities to improve cross-chain compatibility}
 
Interoperability issues between different blockchain platforms are prominent, and cross-chain compatibility of smart contracts is crucial. "[BOOK] Blockchain for business"\cite{36}introduces the application of blockchain technology in the business field. Although it does not directly discuss optimizing LLM's code generation capabilities, it provides background knowledge for understanding cross-chain requirements."Hybrid RAG-empowered Multi-modal LLM for Secure Healthcare Data Management: A Diffusion-based Contract Theory Approach" \cite{37}proposed a multi-modal language model based on hybrid RAG enhancement. Although it mainly focuses on the medical field, the diffusion contract in it Theoretical methods have certain implications for optimizing LLM's code generation capabilities to improve cross-chain compatibility. At the same time, "A survey on blockchain interoperability: Past, present, and future trends"\cite{38}conducted a comprehensive study on the interoperability of blockchain, discussed the interoperability issues between different blockchains and the implementation of cross-chain Methods for communication and data sharing, various interoperability solutions are reviewed, challenges and future research directions are analyzed, and the importance of standardization and cooperation is emphasized. "Application of large language models to software engineering tasks: Opportunities, risks, and implications"\cite{39}discusses the application of large language models in software engineering tasks, including opportunities, risks, and implications, and provides information for optimizing LLM's code generation capabilities. refer to."Large language models for software engineering: A systematic literature review"\cite{40}This systematic literature review studies the application of large language models in software engineering, covering aspects such as code generation, testing, document generation and project management, and analyzes The advantages and limitations are discussed, the practical application effects are discussed, and future research directions are proposed. Researchers explore and optimize its code generation capabilities to adapt to different blockchain platforms, and combine cross-chain technology to achieve seamless migration of smart contracts between different platforms. At present, this field is in the research stage, and it is necessary to solve the generalization ability and adaptability issues of LLM and strengthen the integration with different platforms.
